Macroscopic Resonant Tunneling through Andreev Interferometers

We investigate the conductance through and the spectrum of ballistic chaotic quantum dots attached to two s-wave superconductors, as a function of the phase difference $\phi$ between the two order parameters. A combination of analytical techniques -- random matrix theory, Nazarov's circuit theory and the trajectory-based semiclassical theory -- allows us to explore the quantum-to-classical crossover in detail. When the superconductors are not phase-biased, $\phi=0$, we recover known results that the spectrum of the quantum dot exhibits an excitation gap, while the conductance across two normal leads carrying $N_{\rm N}$ channels and connected to the dot via tunnel contacts of transparency $\Gamma_{\rm N}$ is $\propto \Gamma_{\rm N}^2 N_{\rm N}$. In contrast, when $\phi=\pi$, the excitation gap closes and the conductance becomes $G \propto \Gamma_{\rm N} N_{\rm N}$ in the universal regime. For $\Gamma_{\rm N} \ll 1$, we observe an order-of-magnitude enhancement of the conductance towards $G \propto N_{\rm N}$ in the short-wavelength limit. We relate this enhancement to resonant tunneling through a macroscopic number of levels close to the Fermi energy. Our predictions are corroborated by numerical simulations.

==> bibliography.tex <==
\begin{thebibliography}{99}
\bibitem{And64} A.\ F.\ Andreev, Zh.\ Eksp.\ Teor.\ Fiz.\ {\bf 46}, 1823
  (1964) [Sov.\ Phys.\ JETP {\bf 19} 1228 (1964)].
\bibitem{Imry} Y. Imry, {\it Introductino to Mesoscopic Physics}
(Oxford University, Oxford, 2002); B.J. van Wees and H. Takayanagi, in
{\it Mesoscopic Electron Transport}, L.L. Sohn, L.P. Kouwenhoven 
and G. Sch\"on Eds., NATO ASI Series E345 (Kluwer, Dordrecht, 1997).
\bibitem{Kos95} I.\ Kosztin, D.\ L.\ Maslov, and P.\ M.\ Goldbart, Phys.\
  Rev.\ Lett.\ {\bf 75}, 1735 (1995).
\bibitem{Mel96}  J.\ A.\ Melsen, P.\ W.\ Brouwer, K.\ M.\ Frahm, and C.\ W.\
  J.\ Beenakker, Europhys.\ Lett.\ {\bf 35}, 7 (1996). 
\bibitem{Sch99} H.\ Schomerus and C.\ W.\ J.\ Beenakker, Phys.\ Rev.\ Lett.\
  {\bf 82}, 2951 (1999).
\bibitem{BGS}
O.~Bohigas, M.~J. Giannoni, and C.~Schmit.
Phys. Rev. Lett. {\bf 52}, 1 (1984);
S. M\"uller, S. Heusler, P. Braun P, F. Haake, and A. Altland,
Phys. Rev. Lett. {\bf 93}, 014103 (2004).
\bibitem{Lod98} A.\ Lodder and Yu.\ V.\ Nazarov, Phys.\ Rev.\ B {\bf 58}, 5783 (1998).
\bibitem{Sch05} H. Schomerus and 
Ph. Jacquod, J. Phys. A. {\bf 38}, 10663 (2005).
\bibitem{Vav03} M.\ G.\ Vavilov and A.\ I.\ Larkin, Phys.\ Rev.\ B {\bf 67},
  115335 (2003).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Ehrenfest for Andreev billiards
\bibitem{Ada02} \.{I}.\ Adagideli and C.\ W.\ J.\ Beenakker, Phys.\ Rev.\
  Lett.\ {\bf 89}, 237002 (2002).
\bibitem{Sil03} P.\ G.\ Silvestrov, M.\ C.\ Goorden, and C.\ W.\ J.\
  Beenakker, Phys.\ Rev.\ Lett.\ {\bf 90}, 116801 (2003).
\bibitem{Jac03} Ph.\ Jacquod, H.\ Schomerus, and C.\ W.\ J.\ Beenakker, Phys.\
  Rev.\ Lett.\ {\bf 90}, 207004 (2003).
\bibitem{Goo03} M.\ C.\ Goorden, Ph.\ Jacquod, and C.\ W.\ J.\ Beenakker,
  Phys.\ Rev.\ B {\bf 68} 220501(R) (2003).
\bibitem{Kor04} A. Korm\'anyos, Z. Kaufmann, C.J. Lambert, and J. Cserti, 
Phys.\ Rev.\ B\ {\bf 70}, 052512 (2004).
\bibitem{Goo05} M.\ C.\ Goorden, Ph.\ Jacquod, and C.\ W.\ J.\ Beenakker,
  Phys.\ Rev.\ B {\bf 72}, 064526 (2005).
\bibitem{Silv06} P.G. Silvestrov, Phys. Rev. Lett. {\bf 97}, 067004 (2006). 
%%%%%%%%%%% other Andreev billiards
\bibitem{Mel97}  J.\ A.\ Melsen, P.\ W.\ Brouwer, K.\ M.\ Frahm, and C.\ W.\
  J.\ Beenakker, Physics Scripta {\bf T69}, 223 (1997).

\bibitem{Zho98} F. Zhou, P. Charlat, B. Spivak, and B. Pannetier,
J. Low Temp. Phys. {\bf 110}, 841 (1998).
\bibitem{Tar01} D. Taras-Semchuk and A. Altland, Phys. Rev. B {\bf 64},
014512 (2001).

%%%%%%%%%%%%%% general RMT reference
\bibitem{Bee97} C.\ W.\ J.\ Beenakker, Rev.\ Mod.\ Phys.\ {\bf 69}, 731 (1997).

%%%%%%%%%%%%%%%%%% transport through Josephson junction
\bibitem{Blom} H.A. Blom, A. Kadigrobov, A.M. Zagoskin, R.I. Shekhter, 
and M. Jonson, Phys. Rev. B {\bf 57}, 9995 (1998). In 
this article, the chaoticity of the cavity is related to the strength
of the tunnel barriers between the leads and the cavity in such a way that, 
in the tunneling limit, $\Gamma_{\rm N} \ll 1$, the cavity becomes regular.

\bibitem{Kad95} A. Kadigrobov, A. Zagoskin, R.I. Shekhter, and M. Jonson, 
Phys. Rev. B {\bf 52}, R8662 (1995). This article makes
the unphysical assumption that the interferometer 
does not mix transport modes and therefore acts as $N$ identical 
one-dimensional interferometers in parallel.

\bibitem{Spi82} B.Z. Spivak and D.E. Khmel'nitskii, JETP Lett. {\bf 35}, 412 (1982). This work lies somehow outside our present focus, as it considers 
temperatures larger than $E_{\rm T,S}$.

\bibitem{Zai94} A.V. Zaitsev, Phys. Lett. A {\bf 194}, 315 (1994).

\bibitem{Kad99} A. Kadigrobov, L.Y. Gorelik, R.I. Shekhter, and M. Jonson,
Superlattices and Microstructures {\bf 25}, 961 (1999). 

\bibitem{Bee95} C.W.J. Beenakker, J.A. Melsen, and P.W. Brouwer,
Phys. Rev. B {\bf 51}, 13883 (1995).

%%%%%%%%%%%%%% circuit theory
\bibitem{Naz94} Y.\ V.\ Nazarov, Phys.\ Rev.\ Lett.\ {\bf 73}, 1420 (1994).
\bibitem{Arg96} N.\ Argaman, Europhys.\ Lett.\ {\bf 38}, 231 (1997).

%%%%%%%%%%%%%%%%%%%%%%% more semiclassics
\bibitem{Jac06} Ph.\ Jacquod and R.\ S.\ Whitney, Phys.\ Rev.\ B {\bf 73},
  195115 (2006).

\bibitem{Semicl} K. Richter and M. Sieber, Phys. Rev. Lett. {\bf 89}, 
206801 (2002); 
S. Heusler, S. M\"uller, P. Braun, and F. Haake,
Phys. Rev. Lett. {\bf 96}, 066804 (2006).

\bibitem{Ada03} \.{I}.\ Adagideli, Phys.\ Rev.\ B {\bf 68}, 233308 (2003).

\bibitem{Bro06a} P.\ W.\ Brouwer and S.\ Rahav, Phys.\ Rev.\ B {\bf 74}, 075322 (2006).

\bibitem{Whi07} R.S. Whitney, Phys. Rev. B {\bf 75}, 235404 (2007).

\bibitem{Fra96} K.M. Frahm, P.W. Brouwer, J.A. Melsen, and C.W.J. Beenakker,
Phys. Rev. Lett. {\bf 76}, 2981 (1996).

\bibitem{Zir97} A.\ Altland and M.\ R.\ Zirnbauer, Phys.\ Rev.\ B {\bf 55},
  1142 (1997).

\bibitem{Ihra01} W. Ihra, M. Leadbeater, J.L. Vega, and K. Richter,
Eur. Phys. J. B {\bf 21}, 425 (2001); O. Zaitsev, J. Phys. A {\bf 39}, L467 (2006).

\bibitem{Iida90} S. Iida, H.A. Weidenm\"uller, and J.A. Zuk, Phys. Rev. 
Lett. {\bf 64}, 583 (1990).

%%%%%%%%%%%%%%%%%%%%%%%% transport with superconductivity
\bibitem{Lam93} C.J. Lambert, J. Phys. Cond. Mat. {\bf 5}, 707 (1993);
N.\ R.\ Claughton and C.\ J.\ Lambert, Phys.\ Rev.\ B {\bf
  53}, 6605 (1996).

\bibitem{Cou92} L. Couchman, E. Ott, and T.M. Antonsen,
Phys. Rev. A {\bf 46}, 6193 (1992).

\bibitem{caveat} The segments $\gamma_{si}$, $i=1,2,3$ in 
Fig.\ref{fig:device} might include many intermediate
bounces at a tunnel barrier. All possible number of reflections are 
effectively resummed; see Ref.~\cite{Whi07} for more details.

\bibitem{Haake-book} F.~Haake, {\it Quantum Signatures of Chaos}, 2nd Ed.
Springer, Berlin (2001).

\bibitem{Ket99} R.\ Ketzmerick, K.\ Kruse, and T.\ Geisel, Physics D {\bf
  131}, 247 (1999).

\bibitem{Fyo00} Y.\ V.\ Fyodorov and H.-J.\ Sommers, JETP Lett.\ {\bf 72}, 422
  (2000).

\bibitem{Two03} J.\ Tworzyd{\l}o, A.\ Tajic and C.\ W.\ J.\ Beenakker, Phys.\
  Rev.\ B {\bf 68}, 115313 (2003).

\end{thebibliography}
